SEEK: Semantic Evidence Extraction via Adaptive ChunKing for Multilingual Fact-Checking

Multilingual fact verification requires evidence that is both relevant and sufficiently complete for reliable factuality prediction. However, existing systems often rely on search snippets, sentence-level evidence, or locally segmented passages, which can miss decisive context and produce fragmented evidence. To overcome these limitations, we propose SEEK, a Semantic Evidence Extraction with an adaptive chunKing framework that constructs coherent evidence chunks from full fact-checking articles by identifying semantic topic transitions and preserving local verification context. The constructed chunks are encoded using a multilingual encoder and then multilingual LLMs are finetuned using LoRA adapter for veracity prediction. Experiments on X-FACT and RU22Fact show that SEEK improves macro-f1 by up to 10% over semantic chunking, 19% over sentence chunking, and 20% over search-snippet baselines. Evidence completeness and significance analyses further show that SEEK preserves richer verification context and enables more reliable multilingual fact-checking.

==> tables/evidence_completeness_prompt.tex <==
\begin{table}[ht]
\centering
\small
\begin{tabular}{p{1\columnwidth}}
\toprule
You are evaluating retrieved evidence for a fact-checking task. \\[0.3em]

\textbf{Claim:} \{claim\} \\[0.3em]

\textbf{Retrieved Evidence:} \{evidence\} \\[0.3em]

\textbf{Question:} Does the retrieved evidence contain enough information to verify whether the claim is true or false? \\[0.3em]

Choose exactly one label: \\[0.0em]

\textbf{Complete:} The evidence contains sufficient information to verify the claim. \\

\textbf{Partial:} The evidence is related to the claim but incomplete. \\

\textbf{Irrelevant:} The evidence is unrelated, noisy, empty, blocked webpage text, or does not help verify the claim. \\[0.3em]

Return only one word: \textit{Complete}, \textit{Partial}, or \textit{Irrelevant}. \\
\bottomrule
\end{tabular}
\caption{Prompt used for evidence completeness evaluation.}
\label{tab:evidence_completeness_prompt}
\end{table}

==> tables/hyperparameter.tex <==
\begin{table}[ht]
\centering
\small
\setlength{\tabcolsep}{16pt}
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{ll}
\toprule
\textbf{Hyperparameter} & \textbf{Value} \\
\midrule
Fine-tuning method & LoRA \\
Number of epochs & \texttt{3} \\
LoRA rank & \texttt{8} \\
Retrieved candidates & \texttt{20} \\
Final evidence chunks & \texttt{5} \\
Retrieval method & FAISS dense retrieval \\
Evaluation metric & Macro-F1 \\
\bottomrule
\end{tabular}
\caption{Hyperparameter settings used across experiments.}
\label{tab:hyperparameters}
\end{table}

==> tables/result3.tex <==
% \begin{table*}[!t]
%   \centering
%   \setlength{\tabcolsep}{8pt}
%   \renewcommand{\arraystretch}{1.2}
%   \resizebox{\textwidth}{!}{%
%     \begin{tabular}{l|l|c|c|c}
%       \toprule
%       \textbf{Dataset} & \textbf{Model} & \textbf{precision} & \textbf{recall} & \textbf{macro-f1} \\
%       \midrule
%       \multirow{3}{*}{X-Fact}
%         & Gemma & 47.68 & 44.36 & 45.74 \\
%         & Llama & 47.60 & 44.94 & 45.91 \\
%         & Mistral & 46.22 & 46.11 & 45.86 \\
%         & Qwen & 46.34 & 44.87 & 45.29 \\
%       \midrule
%       \multirow{4}{*}{Ru22fact}
%         & Gemma & 71.09 & 73.95 & 72.26 \\
%         & Llama & 69.77 & 72.82 & 70.69 \\
%         & Mistral & 71.70 & 76.75 & 72.88 \\
%         & Qwen & 69.26 & 73.51 & 70.10 \\
%       \midrule
%     \end{tabular}
%   }
%   \caption{Macro Precision, Recall, and F1 (\%) scores using semantic chunking.}
%   \label{tab:macro_prf1_semantic_chunking}
% \end{table*}







==> tables/ru22fact_dataset_table.tex <==
% \begin{table}[ht]
% \centering

% \begin{tabular}{lcccc}
% \toprule
% \textbf{Language} & \textbf{Train} & \textbf{Dev} & \textbf{Test} & \textbf{Total} \\
% \midrule
% English    & 6,082 & 867 & 1,741 & 8,690 \\
% Chinese    & 1,055 & 152 & 305 & 1,512 \\
% Russian    & 1,621 & 231 & 465 & 3,399 \\
% Ukrainian  & 2,458 & 350 & 704 & 3,512 \\
% \midrule
% \textbf{Total} & 11,217 & 1,600 & 3,216 & 16,033 \\
% \textbf{\#Supported} & \multicolumn{4}{c}{10,081} \\
% \textbf{\#Refuted} & \multicolumn{4}{c}{4,651} \\
% \textbf{\#NEI} & \multicolumn{4}{c}{1,301} \\
% \bottomrule
% \end{tabular}
% \caption{Statistics of RU22Fact~\cite{zeng2024ru22fact}.}
% \label{tab:ru22fact_statistics}
% \end{table}

\begin{table}[htbp]
\centering
\begin{tabular}{|l|r|r|r|r|}
\hline
\multicolumn{5}{|c|}{\textbf{RU22Fact Label-wise Distribution}} \\
\hline
\textbf{Label} & \textbf{Train} & \textbf{Dev} & \textbf{Test} & \textbf{Total} \\
\hline
Supported & 6,836 & 1,079 & 2,166 & 10,081 \\
Refuted   & 3,299 &   450 &   902 & 4,651 \\
NEI       & 1,082 &    71 &   148 & 1,301 \\
\hline
\textbf{Total} & 11,217 & 1,600 & 3,216 & 16,033 \\
\hline
\end{tabular}
\caption{Label-wise statistics of the RU22Fact dataset~\cite{zeng2024ru22fact}. NEI = Not Enough Information.}
\label{tab:ru22fact_label_statistics}
\end{table}


==> tables/xfact_dataset_table.tex <==
% \begin{table}[htbp]
% \centering
% \setkeys{Gin}{keepaspectratio}
% \resizebox*{0.5\textwidth}{!}{
% \begin{tabular}{|p{2cm}|r|r|r|r|r|r|}
% \hline
% \multicolumn{7}{|c|}{\textbf{X-Fact Dataset} Label Distribution} \\ \hline
% \textbf{Class} & \textbf{Train} & \textbf{Dev} & \textbf{Indomain} & \textbf{OOD} & \textbf{Zeroshot} & \textbf{Total} \\ \hline
% False & 7,515 & 977 & 1,464 & 1,109 & 1,471 & 12,536 \\
% PT/M & 4,359 & 553 & 858 & 769 & 772 & 7,311 \\
% True & 4,080 & 551 & 851 & 329 & 332 & 6,143 \\
% MT& 1,380 & 194 & 300 & 0 & 73 & 1,947 \\
% MF & 848 & 114 & 159 & 0 & 415 & 1,536 \\
% C/H & 540 & 80 & 106 & 150 & 264 & 1,140 \\
% Other & 357 & 66 & 88 & 11 & 54 & 576 \\ \hline
% \textbf{Total} & 19,079 & 2,535 & 3,826 & 2,368 & 3,381 & 31,189 \\ \hline
% \end{tabular}
% }
% \caption{Label-wise distribution across X-Fact dataset splits: Train, Dev, Indomain, Out-of-Domain (OOD), and Zeroshot. Label abberivations: PT/M = Partialy true/Misleading, MT = Mostly true, MF = Mostly false, C/H = Complicated/Hard to categorize }
% \label{tab:xfact_label_distribution}
% \end{table}
\begin{table}[htbp]
\centering
\setkeys{Gin}{keepaspectratio}
\resizebox*{0.5\textwidth}{!}{
\begin{tabular}{|p{1cm}|r|r|r|r|r|r|}
\hline
\multicolumn{7}{|c|}{\textbf{X-Fact Dataset} Label Distribution} \\ \hline
\textbf{Class} & \textbf{Train} & \textbf{Dev} & \textbf{Indomain} & \textbf{OOD} & \textbf{Zeroshot} & \textbf{Total} \\ \hline
False & 7,515 & 977 & 1,464 & 1,109 & 1,471 & 12,536 \\
PT/M & 4,359 & 553 & 858 & 769 & 772 & 7,311 \\
True & 4,080 & 551 & 851 & 329 & 332 & 6,143 \\
MT& 1,380 & 194 & 300 & 0 & 73 & 1,947 \\
MF & 848 & 114 & 159 & 0 & 415 & 1,536 \\
C/H & 540 & 80 & 106 & 150 & 264 & 1,140 \\
Other & 357 & 66 & 88 & 11 & 54 & 576 \\ \hline
\textbf{Total} & 19,079 & 2,535 & 3,826 & 2,368 & 3,381 & 31,189 \\ \hline
\end{tabular}
}
\caption{Label-wise distribution across X-Fact dataset splits. Label abberivations: OOD = Out-of-domain, PT/M = Partialy true/Misleading, MT = Mostly true, MF = Mostly false, C/H = Complicated/Hard to categorize }
\label{tab:xfact_label_distribution}
\end{table}
